Refactoring Delta-Oriented Product Lines to achieve Monotonicity

Delta-oriented programming (DOP) is a flexible transformational approach to implement software product lines. In delta-oriented product lines, variants are generated by applying operations contained in delta modules to a (possibly empty) base program. These operations can add, remove or modify named elements in a program (e.g., classes, methods and fields in a Java program). This paper presents algorithms for refactoring a delta-oriented product line into monotonic form, i.e., either to contain add and modify operations only (monotonic increasing) or to contain remove and modify operations only (monotonic decreasing). Because of their simpler structure, monotonic delta-oriented product lines are easier to analyze. The algorithms are formalized by means of a core calculus for DOP of product lines of Java programs and their correctness and complexity are given.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{Julia Rubin and Thomas Th\"um (Eds.):\\
7th International Workshop on Formal Methods and Analysis\\ in Software Product Line Engineering (FMSPLE'16)\\
EPTCS 206, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.206.2}{10.4204/EPTCS.206.2}}

